Sharp bounds of constants in Poincare type inequalities for polygonal domains

The paper is concerned with sharp estimates of constants in Poincare type inequalities for functions having zero mean value on the boundary of a Lipschitz domain or on a measurable part of it. These estimates are useful for various numerical methods, in particular, for a posteriori error estimation methods for partial differential equations (PDEs). Therefore, we are mainly focused on domains typical for numerical analysis (simplexes in 2d and 3d) and suggest easily computable relations that provide sharp bounds of the respective constants. Also, we investigate numerically the behavior of the constants in the classical Poincare inequalities and compare these results with known analytical estimates. In the last section, the estimates are used in order to obtain new a posteriori estimates for an elliptic boundary value problem.

==> 2d-simplex.tex <==
\begin{tikzpicture}[remember picture]

% coordinate axis Ox
\draw[->] (0.0, 0.0) -- (3.1, 0.0) node[anchor=west] {$x_1$};
\draw[->] (0.0, 0.0) -- (0.0, 4.0) node[anchor=west] {$x_2$};

% another triangle
\draw (0,0) node[anchor=north east] {$A (0, 0)$} --
      (2.8,0) node[anchor=north west] {$B (h, 0)$} --
      (1.8,2.5)  node[anchor=south west]
            {$C \big(h \rho \cos\alpha, h \rho \sin\alpha \big)$}-- (0,0);


\filldraw [black] (0,0) circle (0.8pt)
                  (2.8,0) circle (0.8pt)
                  (1.8,2.5) circle (0.8pt);

\draw (0.4,0.0) .. controls (0.3,0.3) and (0.2, 0.3) .. (0.2,0.3);
\draw (0.5,0.1) node[anchor=south] {$\alpha$};

\draw (1.5,0.5) node[anchor=west] {$T$};
\draw [ultra thick] (0,0) -- (2.8,0);
\draw (2,-1.0) node[anchor=south] {${\Gamma}$};
\end{tikzpicture}


==> 3d-simplex.tex <==
\begin{tikzpicture}[remember picture]

%\coordinate [label=above right: $\widehat{\mathrm{A}}$] (A) at (0,0,0);
%\coordinate [label=above right:$\widehat{\mathrm{B}}$] (B) at (2,0,0);
%\draw (2.3, -0.1, 0) node[anchor=south west] {$(1, 0, 0)$};
%\coordinate [label=below:$\widehat{\mathrm{C}}$] (C) at (0,0,2);
%\draw (1.5, -0.07, 2) node[anchor=north east] {$(0, 0, 1)$};
%\coordinate [label=above right:$\widehat{\mathrm{D}}$] (D) at (0,2,0);
%\draw (0.35, 2.52, 0) node[anchor=north west] {$(0, 1, 0)$};
%
%\draw[->] (2,0, 0) -- (3.5,0,0) node[right] {$\hat{x}_1$};
%\draw[->] (0,2, 0) -- (0,3,0) node[above] {$\hat{x}_2$};
%\draw[->] (0,0, 2) -- (0,0,3) node[below left] {$\hat{x}_3$};
%
%\draw (1.3, 1.1) node[anchor=north east] {$\Tref_{\rfrac{\pi}{2}, \rfrac{\pi}{2}}$};
%\draw (1.2, -0.4) node[anchor=north east] {$\widehat{\Gamma}$};
%
%\draw[-, fill=black!10, opacity=.5, dashed] (A)--(B)--(C)--(A);
%\draw[-, opacity=.5] (B)--(C);
%\draw[-, opacity=.5] (C)--(D);
%\draw[-, opacity=.5] (B)--(D);
%
%\draw[dashed] (A)--(D);
%
%\draw[->] (1.8,1.8) .. controls (2.2,2.2) and (3.5,3) .. node[above] {$\mathcal{F}_{\theta, \alpha}$} (4.5,2);

\coordinate [label=above right:$$] (B) at (9,0,0);
\coordinate [label=below:$$] (C) at (5,0,4.5);
\coordinate [label=above left:$$] (D) at (6.5,3,2);
\coordinate [label=above left:$$] (N) at (6.5,3,0);
\coordinate [label=above:$$] (M) at (6.5,0,0);
\coordinate [label=below:$$] (H) at (6.6,0,2);
\coordinate [label=below:$$] (L) at (5,3,2);
\coordinate [label=below:$$] (O) at (5,0,2);

\coordinate [label=below:A] (A) at (5,0,0);
\draw[-, fill=black!10, opacity=.5, dashed] (A)--(B)--(C)--(A);

\coordinate [label=below:A] (A) at (5,0,0);

%
\draw (6.4, 1.2, 1) node[anchor=north west] {$\T_{\theta, \alpha}$};
\draw (7, -0.1) node[anchor=north east] {${\Gamma}$};

\draw[->] (8.5,0,0) -- (9.5,0,0) node[right] {$x_1$};
\draw[->] (5,0,0) -- (5,3,0) node[above] {$x_2$};
\draw[->] (C) -- (5,0,5.5) node[below] {$x_3$};
%
\draw[->] (4.8,-0.2) .. controls (4.9, 0.4) and (5, 0.5) .. node[right] {$$}  (5.2, 0.7);
%\draw (4.85,-0.15) .. controls (4.85, 0.45) and (4.95, 0.45) .. node[right] {$$}  (5.11, 0.55);
\draw (4.9, 0.5) node[anchor=north east] {$\theta$};
\draw (5,0.01,5) node[anchor=north west] {$C (0, 0, h_3)$};
\draw (8.0,0.01,0) node[anchor=north west] {$B (h_1, 0, 0)$};
\draw (6.2,3,2) node[anchor=south west] {$D$};

\draw[->] (5.5,0.0) .. controls (5.4, 0.3) and (5.3, 0.4) .. node[right] {$\alpha$}  (5.23,0.47);

\draw[-, opacity=.5] (A)--(D);
\draw[-, opacity=.5] (B)--(C);
\draw[-, opacity=.5] (C)--(D);
\draw[-, opacity=.5] (B)--(D);
\draw[dashed] (D)--(H);
%\draw[-] (5.8,0,1.5)--(5.8,0.2,1.5)--(6,0.2,1.5);
%\draw[dashed] (5.5, 0.0,1.5)--(6.5,0.0,1.5);
\draw[dashed] (A)--(H);
\draw[dashed] (H)--(M);
\draw[dashed] (N)--(M);
\draw[dashed] (N)--(B);
\draw[dashed] (N)--(D);
\draw[dashed] (N)--(A);
%\draw[dashed] (L)--(D);
\draw[dashed] (H)--(O);
\draw[dashed] (D)--(O);

%\draw[-] (5.8,0,1.5)--(5.8,0.2,1.5)--(6,0.2,1.5);
%\draw[dashed] (5.5, 0.0,1.5)--(6.5,0.0,1.5);

% pi/2 angle 
%\draw[-] (5,0,2.6)--(5,0.3,2.1)--(5,0.3,1.3);

%
\foreach \i in {B,C}
    \draw[dashed] (A)--(\i);
%

\filldraw [black] (4.5,0,0) circle (0.8pt)
                  (9,0,0) circle (0.8pt)
                  (5,0,5) circle (0.8pt)
									(6.5,3,2) circle (0.8pt);


\end{tikzpicture}



==> cp-with-estimates-comparison.tex <==
%********************************************************************************************
%rho = 0.7, 0.86, 1, 1.5
%********************************************************************************************
\begin{figure}[!ht]
	\centering
	\subfloat[$\rho = \tfrac{\sqrt{2}}{2}$]{
	\includegraphics[scale=0.8]{2d-cp-mean-value-on-T-comparison-LS-MR-rho-0-70711-h-1-1-power-series}	\label{fig:cp-rho-sqrt2-2}
	}\\[-1pt]
	\subfloat[$\rho = \tfrac{\sqrt{3}}{2}$]{
	\includegraphics[scale=0.8]{2d-cp-mean-value-on-T-comparison-LS-MR-rho-0-86603-h-1-1-power-series}	\label{fig:cp-rho-sqrt3-2}
	}\\[-1pt]
	\subfloat[$\rho = 1$]{
	\includegraphics[scale=0.8]{2d-cp-mean-value-on-T-comparison-LS-MR-rho-1-h-1-1-power-series}
	\label{fig:cp-rho-1}}\\[-2pt]
	\subfloat[$\rho = \tfrac{3}{2}$]{
	\includegraphics[scale=0.8]{2d-cp-mean-value-on-T-comparison-LS-MR-rho-1-5-h-1-1-power-series}
	\label{fig:cp-rho-3-2}
	}\\[0pt]
	\subfloat[$\rho = 2$]{
	\includegraphics[scale=0.8]{2d-cp-mean-value-on-T-comparison-LS-MR-rho-2-h-1-1-power-series}
	\label{fig:cp-rho-2}
	}
	\caption{$\underline{C}^{48}_{\T}$ with upper bounds $\CPLS$ and $\CPMR$ and lower bound 
	with respect to $\alpha$ on $\T$ with (a) $\rho = \tfrac{\sqrt{2}}{2}$, (b) $\tfrac{\sqrt{3}}{2}$, (c) $1$, (d) $\tfrac{3}{2}$, and (e) $2$.}	
	\label{fig:2d-cp-rho}
\end{figure}



==> cp-with-estimates-small.tex <==
%********************************************************************************************
%rho = 0.71, 1.5
%********************************************************************************************
\begin{figure}[!ht]
	\centering
	\subfloat[$\rho = \tfrac{\sqrt{2}}{2}$]{
	\includegraphics[scale=0.8]{2d-cp-mean-value-on-T-rho-0-70711-h-1-1-power-series}
	\label{fig:cp-rho-sqrt2-2}}\\
	\subfloat[$\rho = 1$]{
	\includegraphics[scale=0.8]{2d-cp-mean-value-on-T-rho-1-h-1-1-power-series}
	\label{fig:cp-rho-1}} \\
	\subfloat[$\rho = \tfrac{3}{2}$]{
	\includegraphics[scale=0.8]{2d-cp-mean-value-on-T-rho-1-5-h-1-1-power-series}
	\label{fig:cp-rho-3-2}
	}
	\caption{$\underline{C}^{48}_{\T}$ with upper and lower bounds 
	with respect to $\alpha$ on $\T$ with (a) $\rho = \tfrac{\sqrt{2}}{2}$ and (b) $\tfrac{3}{2}$.}	
	\label{fig:2d-cp-rho}
\end{figure}

\begin{figure}[!ht]
  \centering
	\includegraphics[scale=0.8]{2d-cp-mean-value-on-T-improved-rho-1-h-1-1-power-series}
	\captionof{figure}{Approximation $\underline{C}^{48}_{\T}$ with improved upper and 
	lower bounds on isosceles $\T$ with respect to $\alpha$.}
	\label{fig:cp-rho-1-improved}
\end{figure}


==> cpgamma-ctrgamma-with-estimates-ref-case-small.tex <==
%-------------------------------------------------------------------------------------------%
% \CPT with upper bounds
%--------------------------------------------------------------------------------------------%

\begin{figure}[!ht]
	\centering
	\subfloat[$\rho = \tfrac{\sqrt{2}}{2}$]{
  \includegraphics[scale=0.85]{exact-and-approx-C-PT-rho-0-70711-h-1-1-power-series}
	\label{fig:2d-cpt-rho-sqrt2-2}}
	\quad
	\subfloat[$\rho = \tfrac{\sqrt{2}}{2}$]{
	\begin{tikzpicture}[thick, scale=0.9]
	\draw[dashed] (2.1213,0) arc (0:180:2.1213cm);

	% coordinate axis Ox
	\draw[->] (0.0, 0.0) -- (3.5, 0.0) node[anchor=west] {$x_1$};
	\draw[->] (0.0, 0.0) -- (0.0, 3.5) node[anchor=west] {$x_2$};

	% another triangle
	\draw (0.0,0.0) node[anchor=north east] {$(0, 0)$} --
				(2.1213,0.0) node[anchor=north west] {$(1, 0)$} --
				(0.0,2.1213)  node[anchor=south west] {$(0, 1)$}-- (0,0);

	\filldraw [black] (0.0,0.0) circle (0.8pt)
										(2.1213,0.0) circle (0.8pt)
										(0.0,2.1213) circle (0.8pt);

	\draw (0,0.2) -- (0.2,0.2) -- (0.2, 0); 
	\draw (0.4, -0.6) node[anchor=south] {$\tfrac{\pi}{2}$};
	
	\draw [ultra thick] (0,0) -- (3,0); 
	\draw (1.5,-0.8) node[anchor=south] {${\Gamma}$};
	
	%---------------------------------------------------------------%
	
	\draw [ultra thick](0.0,0.0) -- (3.0, 0.0) -- (1.5, 1.5) -- (0,0);
	
	\filldraw [black] (0.0,0.0) circle (0.8pt)
										(3.0,0.0) circle (0.8pt)
										(1.5, 1.5) circle (0.8pt);
	\draw (1.0,0.0) .. controls (1.0,0.2) and (0. 95, 0.5) .. node[right] {$\tfrac{\pi}{4}$}  (0.8,0.72);

	%---------------------------------------------------------------%

	\draw (0.0,0.0) -- (3.0, 0.0) -- (1.0607, 1.8371) -- (0,0);
	
	\filldraw [black] (0.0,0.0) circle (0.8pt)
										(3.0,0.0) circle (0.8pt)
										(1.0607, 1.8371) circle (0.8pt);
	\draw (0.8, 0.0) .. controls (0.8, 0.4) and (0.7, 0.58) .. node[anchor=south] {$ $}  (0.49,0.82);
  \draw (0.3, 0.6) node[anchor=south] {$\tfrac{\pi}{3}$};
	
	%---------------------------------------------------------------%

	\draw (0.0,0.0) -- (3.0, 0.0) -- (-1.0607, 1.8371) -- (0,0);
	
	\filldraw [black] (0.0,0.0) circle (0.8pt)
										(3.0,0.0) circle (0.8pt)
										(-1.0607, 1.8371) circle (0.8pt);
	\draw (0.6, 0.0) .. controls (0.6,0.7) and (-0.1, 0.9) .. node[anchor=south] {$ $}  (-0.4,0.7);
  \draw (-0.2, 0.7) node[anchor=south] {$\tfrac{2\pi}{3}$};
	
	\end{tikzpicture}
	\label{eq:t-rho-sqrt2-2}
 	}\\
	\subfloat[$\rho = 1$]{
  \includegraphics[scale=0.85]{exact-and-approx-C-PT-rho-1-h-1-1-power-series}
	\label{fig:2d-cpt-rho-1}}
	\; \;
	\subfloat[$\rho = 1$]{
  \begin{tikzpicture}[thick, scale=0.8]

	\draw[dashed] (3,0) arc (0:180:3cm);

	% coordinate axis Ox
	\draw[->] (0.0, 0.0) -- (3.2, 0.0) node[anchor=west] {$x_1$};
	\draw[->] (0.0, 0.0) -- (0.0, 3.5) node[anchor=west] {$x_2$};

	% another triangle
	\draw[ultra thick] (0.0,0.0) node[anchor=north east] {$(0, 0)$} --
				(3.0,0.0) node[anchor=north west] {$(1, 0)$} --
				(0.0,3.0)  node[anchor=east] {$(0, 1)$}-- (0,0);


	\filldraw [black] (0.0,0.0) circle (0.8pt)
										(3.0,0.0) circle (0.8pt)
										(0.0,3.0) circle (0.8pt);

	\draw (0,0.2) -- (0.2,0.2) -- (0.2, 0); 
	\draw (0.4, -0.6) node[anchor=south] {$\tfrac{\pi}{2}$};
	
	\draw [ultra thick] (0,0) -- (3,0); 
	\draw (1.5,-0.8) node[anchor=south] {${\Gamma}$};
	
	%---------------------------------------------------------------%
	
	\draw (0.0,0.0) -- (3.0, 0.0) -- (2.5981,1.5) -- (0,0);
	
	\filldraw [black] (0.0,0.0) circle (0.8pt)
										(3.0,0.0) circle (0.8pt)
										(2.5981,1.5) circle (0.8pt);
	\draw (1.0,0.0) .. controls (1.0,0.2) and (0. 95, 0.4) .. node[right] {$\tfrac{\pi}{6}$}  (0.89,0.5);

	%---------------------------------------------------------------%

	\draw (0.0,0.0) -- (3.0, 0.0) -- (1.5,2.5981) -- (0,0);
	
	\filldraw [black] (0.0,0.0) circle (0.8pt)
										(3.0,0.0) circle (0.8pt)
										(1.5,2.5981) circle (0.8pt);
	\draw (0.8, 0.0) .. controls (0.8,0.4) and (0.7, 0.58) .. node[anchor=south] {$ $}  (0.49,0.82);
  \draw (0.78, 0.6) node[anchor=south] {$\tfrac{\pi}{3}$};
	
	%---------------------------------------------------------------%

	\draw (0.0,0.0) -- (3.0, 0.0) -- (-1.5,2.5981) -- (0,0);
	
	\filldraw [black] (0.0,0.0) circle (0.8pt)
										(3.0,0.0) circle (0.8pt)
										(-1.5,2.5981) circle (0.8pt);
	\draw (0.6, 0.0) .. controls (0.6,0.7) and (-0.1, 0.9) .. node[anchor=south] {$ $}  (-0.4,0.7);
  \draw (-0.2, 0.7) node[anchor=south] {$\tfrac{2\pi}{3}$};
	
	\end{tikzpicture}
	\label{eq:t-rho-1}}
	\caption{Lower and upper bounds  of $\CPT$
	%$\CP = \min \,\{ {\CP}_{\rm I}, {\CP}_{\rm II} \}$ 
	for $\T \in \Rtwo$ (a)-(b) 
	$\rho = \tfrac{\sqrt{2}}{2}$ and (c)-(d) $\rho = 1$.}
	\label{fig:2d-cpt}
\end{figure}
%
\vskip -10pt
%--------------------------------------------------------------------------------------------%
% \CGT with upper bounds
%--------------------------------------------------------------------------------------------%
\begin{figure}[!ht]
	\centering
	\subfloat[$\rho = \tfrac{\sqrt{2}}{2}$]{
  \includegraphics[scale=0.85]{exact-and-approx-C-GT-rho-0-70711-h-1-1-power-series}
	\label{fig:2d-cgt-rho-sqrt2-2}}
	\\
	\subfloat[$\rho = 1$]{
  \includegraphics[scale=0.85]{exact-and-approx-C-GT-rho-1-h-1-1-power-series}
	\label{fig:2d-cgt-rho-1}}
	\caption{Lower and upper bound of $\CGT$
	%$\approxCGT$ and upper bound 
	%$\CG = \min \,\{ {\CG}_{\rm I}, {\CG}_{\rm II} \}$, 
	for $\T \in \Rtwo$ (a) $\rho = \tfrac{\sqrt{2}}{2}$ and (b) $\rho = 1$.}
	\label{fig:2d-cgt}
\end{figure}



==> cpgamma-ctrgamma-with-estimates-small.tex <==
%-------------------------------------------------------------------------------------------%
% \CPT with upper bounds
%--------------------------------------------------------------------------------------------%

\begin{figure}[!ht]
	\centering
	\subfloat[$\rho = \tfrac{\sqrt{3}}{2}$]{
  \includegraphics[scale=0.95]{exact-and-approx-C-PT-rho-0-86603-h-1-1-power-series}
	%\includegraphics[scale=0.95]{exact-and-approx-C-PT-rho-1-h-1-1-power-series}
	\label{fig:2d-cpt-rho-sqrt3-2}}
	\quad
	\subfloat[$\rho = \tfrac{3}{2}$]{
	\includegraphics[scale=0.95]{exact-and-approx-C-PT-rho-1-5-h-1-1-power-series}
	\label{fig:2d-cpt-rho-3-2}}
	\caption{Lower and upper bounds  of $\CPT$
	%$\CP = \min \,\{ {\CP}_{\rm I}, {\CP}_{\rm II} \}$ 
	for $\T \in \Rtwo$ (a) $\rho = \tfrac{\sqrt{3}}{2}$ and (b) $\rho = \tfrac{3}{2}$.}
	\label{fig:2d-cpt-no-ref}
\end{figure}
%
\vskip -10pt
%--------------------------------------------------------------------------------------------%
% \CGT with upper bounds
%--------------------------------------------------------------------------------------------%
\begin{figure}[!ht]
	\centering
	\subfloat[$\rho = \tfrac{\sqrt{3}}{2}$]{
  \includegraphics[scale=0.95]{exact-and-approx-C-GT-rho-0-86603-h-1-1-power-series}
	%\includegraphics[scale=0.95]{exact-and-approx-C-GT-rho-1-h-1-1-power-series}
	\label{fig:2d-cgt-rho-sqrt3-2}}
	\quad
	\subfloat[$\rho = \tfrac{3}{2}$]{
	\includegraphics[scale=0.95]{exact-and-approx-C-GT-rho-1-5-h-1-1-power-series}
	\label{fig:2d-cgt-rho-3-2}}
	\caption{Lower and upper bounds  of $\CGT$
	%$\CP = \min \,\{ {\CP}_{\rm I}, {\CP}_{\rm II} \}$ 
	for $\T \in \Rtwo$ (a) $\rho = \tfrac{\sqrt{3}}{2}$ and (b) $\rho = \tfrac{3}{2}$.}
	\label{fig:2d-cgt-no-ref}
\end{figure}
%
